CNN Features off-the-shelf: an Astounding Baseline for Recognition

Recent results indicate that the generic descriptors extracted from the convolutional neural networks are very powerful. This paper adds to the mounting evidence that this is indeed the case. We report on a series of experiments conducted for different recognition tasks using the publicly available code and model of the \overfeat network which was trained to perform object classification on ILSVRC13. We use features extracted from the \overfeat network as a generic image representation to tackle the diverse range of recognition tasks of object image classification, scene recognition, fine grained recognition, attribute detection and image retrieval applied to a diverse set of datasets. We selected these tasks and datasets as they gradually move further away from the original task and data the \overfeat network was trained to solve. Astonishingly, we report consistent superior results compared to the highly tuned state-of-the-art systems in all the visual classification tasks on various datasets. For instance retrieval it consistently outperforms low memory footprint methods except for sculptures dataset. The results are achieved using a linear SVM classifier (or $L2$ distance in case of retrieval) applied to a feature representation of size 4096 extracted from a layer in the net. The representations are further modified using simple augmentation techniques e.g. jittering. The results strongly suggest that features obtained from deep learning with convolutional nets should be the primary candidate in most visual recognition tasks.

==> 3-Result.tex <==
\section{Result}
Bla Bla Bla!

\input{3-1-Classification.tex}
\input{3-2-Fine-grained.tex}
\input{3-3-Retrieval.tex}


==> Attribute_m.tex <==
Multiple labels (attributes) can be assigned to each training sample. Thus, we adopt a one-versus-all approach as explained in section \ref{sec:class_method}. The penalty cost is set to $C$=3. 


==> Classification_m.tex <==
\paragraph{Object classification.} The Pascal VOC object image
classification dataset includes multiple labels for each image and the
standard evaluation measure is the average precision (AP) over the
precision recall (PR) curve. Therefore we adopt a one-versus-all
classification regime. We use a standard unconstrained optimization
formulation, equation (\ref{eq:svm}), of the linear SVM to train an
individual linear classifier for each class from binary labelled
training data $\{(\mathbf{x}_i, y_i)\}$:
\begin{align}
\label{eq:svm}
\underset{\mathbf{w}}{\text{minimize}}\,\,\frac{1}{2}\|\mathbf{w}\|^2+C\sum_i\text{max}(1-y_i\mathbf{w}^T\mathbf{x}_i,0)
\end{align}
When training an SVM for one class we used all the images containing
an instance of that class as the positive samples and the rest as
negative samples. We used libsvm \cite{libsvm} with the trade-off
parameter set to $C$=5 for all classes and chosen by cross-validation
on the training set. Additionally, we augmented the set of positive
samples by mirroring the positive images. We also expanded the set of
negative images by adding the mirror and 2$\times$2 sub-windows of
each negative image to the set. This helps the classification by a
margin of $5\%$ in mAP.
%% Here we use a standard linear SVM (\ref{eq:svm}) to train an individual model for each class. In the training of a class we use all the images containing that class as positive samples and the rest as negative samples. We used libsvm \cite{libsvm} with the trade-off parameter $C=5$ for all classes. This was chosen by cross validation on the training set. Furthermore, we increased the set of positive samples by mirroring the positive images. We also expanded the set of negative images by adding the mirror and 2$\times$2 sub-windows of negative images to the set. This helps the classification with a margin of $5\%$ in mAP.

\paragraph{Scene classification.} Images from the MIT indoor dataset
are labelled with only one semantic class. The standard measure on
this dataset is the mean of the confusion matrix's diagonal
elements. To perform the multi-class classification we use a
one-against-one approach and train $K(K-1)/2$ SVM binary classifiers,
where $K$ is the number of classes. A simple voting procedure
then determines the winning class. We have trained individual SVMs with
$C$=1 for this experiment. It should be noted that we tried a
structured SVM formulation of multi-class SVM using the SVMstruct
package \cite{svm-struct}, but the one-against-one approach performs
better.

%These two facts promotes the effectiveness of multi-class structure SVM formulation since it will jointly optimize for all the classes and is more aligned with mean accuracy measure (as opposed to AP). For this purpose we use the SVMstruct \cite{svm-struct} implementation of structured SVM. We used zero-one loss for misclassification of samples and L2 regularization
% and linear feature mapping. 
%
%\begin{align}
%\label{eq:svmstruct}
%&\underset{\mathbf{w},\mathbf{\xi}}{\text{minimize}}\,\,\frac{1}{2}\|\mathbf{w}\|^2+\frac{C}{n}\sum_{i=1}^{n}\xi_i\\
%\nonumber &\text{s.t.} \quad \forall{i},\xi_i\geq0 \quad \forall{i}, \forall{y}\in \mathbf{Y}\setminus y_i : \mathbf{w}^T \Phi(x_i, y) \geq 1-\xi_i
%\end{align}
%
%Where $\mathbf{Y}$ is the set of all class labels. $\Phi(x,y)$ zero pads the x feature vector according to the class $y$. The trade-off parameter in (\ref{eq:svmstruct}) is set to $C=1$. We further set the tolerance termination criterion $\epsilon=1e-8$. The single slack method and cutting plane \cite{Joachims09} is used as the solver.


==> Finegrained_m.tex <==
There is a single label associated to each bird and flower image in
this dataset and the standard evaluation procedure is by measuring the
mean accuracy. This is aligned with that of MIT-67 indoor dataset so
we use the same classification and training procedure as for the scene
recognition experiments, section \ref{sec:class_method}. The penalty
cost used for the CUB dataset is $C$=3 and $C$=8 for the Oxford 102
flowers dataset. These parameters were optimized using a small subset of
each dataset.


==> retrieval_c.tex <==

%% So far in this paper we have shown that CNN-representations with simple distance metric can outperform most of the state of the art techniques in classic computer vision scenarios. 
%% To provide a fair comparison, we show a case where this simple solution fails to compete with classic computer vision solutions.
%% \paragraph{Rotation invariance image retrieval}
%% This paper's result shows that CNN-representation can handle camera rotation alongside X and Y axis very well mainly because of pooling layers in computing the representations. But in-plane rotation of images axis totally changes the outcome of first layer and with it, the final representation. figure \ref{fig:retievalRotation} shows the effect of the rotation of query images on the performance of CNN-representation and VLAD \cite{Arandjelovic13}.
\begin{figure}
\begin{center}
\includegraphics[clip=true, trim=0cm 7.5cm 0cm 7cm, width=0.9\linewidth]{Graphics/retrieval/oxROT.pdf}
\end{center}
\vspace{-0.5cm}
\caption{The effect of rotation of query images on the retrieval results over Oxford5k}
\label{fig:retievalRotation}
\end{figure}

%% The simple solution of equation \ref{eq:rotSimilarity} only achieves the mAP of 0.429 while rotating the query images to it's correct angle provides mAP of 0.522.
%% All in all, even though the simple CNN-representation outperforms many of the current state of the art classic computer vision pipelines, in-plane rotation seems to be the Achilles heel for our straight forward solutions.
%% \begin{equation}
%% sim(Im_q,Im_r) = \max\limits_{\theta=0}^{2\pi} sim(rotate(Im_q,\theta),Im_r)
%% \label{eq:rotSimilarity}
%% \end{equation}

